Hybridization of lattice and charge order excitations in a superconducting cuprate

The ubiquitous tendency of superconducting cuprates to form charge density waves (CDWs) has reignited interest in the nature of their electron-phonon interaction and its role in shaping their phase diagrams. While pronounced dispersion anomalies were reported in several phonon branches, their precise connection to charge order and superconductivity remains unresolved. Here, using high-resolution inelastic x-ray scattering under low temperature and high magnetic field, we uncover a striking phonon renormalization in YBa$_2$Cu$_3$O$_{6+x}$. It appears along a reciprocal space trajectory connecting the wave vectors of a short-range 2D-CDW, emerging above the superconducting transition, and a long-range 3D-CDW, appearing only when superconductivity is strongly suppressed. The spectral changes are strongest around the wave vector of the 3D-CDW despite the fact that it is absent in our experimental conditions. Our findings challenge conventional phonon self-energy renormalization models, instead support a scenario in which low-energy phonons hybridize with dispersive CDW excitations and provide insights into the interplay between lattice vibrations and electronic correlations in high-temperature superconductors.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne '') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
